Real-time Curative Actions for Power Systems via Online Feedback Optimization

Curative or remedial actions are the set of immediate actions intended to bring the power grid to a safe operating point after a contingency. The effectiveness of these actions is essential to guarantee curative N-1 security. Nowadays, curative actions are derived ahead of time, based on the anticipated future grid state. Due to the shift from steady to volatile energy resources, the grid state will frequently change and the curative actions would need to be pre-planned increasingly often. Furthermore, with the shift from large bulk production to many small decentralized energy sources more devices need to be actuated simultaneously to achieve the same outcome. Instead of pre-planning, we propose to calculate these complex curative actions in real-time after the occurrence of a contingency. We show how the method of Online Feedback Optimization (OFO) is well suited for this task. As a preliminary demonstration of these capabilities, we use an (OFO) controller, that after a fault, reduces the voltage difference over a breaker to enable the operators to reclose it. This test case is inspired by the 2003 Swiss-Italian blackout, which was caused by a relatively minor incident followed by ineffective curative actions. Finally, we identify and discuss some open questions, including closed-loop stability and robustness to model mismatch.

==> 2023_PowerTech_Emergency Power System Operations via Online Feedback Optimization/figures/block_diagram_AGC.tex <==
\begin{figure}[h]
    \center
    \begin{adjustbox}{width=\columnwidth}
    \begin{tikzpicture}
        \draw[stealth-] (0,0.5) to (-.5,0.5) node[left] {$\Delta \bar \omega$};
        \draw (0,0) rectangle +(1.5,1) node[pos=.5] {$-\lambda$};
        \draw[-stealth] (1.5,0.5) to (2,0.5);
        \draw (2,0) rectangle +(1.5,1) node[pos=.5] {$\frac{K_i + s K_p}{s}$};
        \draw[-stealth] (3.5,0.5) to (4,0.5);
        \draw (4,0) rectangle +(1.5,1) node[pos=.5] {$\bm\beta$};
        \draw[-stealth] (5.5,0.5) to (6,0.5) node[right] {$\bm p_{AGC}$};
    \end{tikzpicture}
    \end{adjustbox}
    \caption{Block diagram of the automated generation control.}
    \label{fig:AGC}
\end{figure}

==> 2023_PowerTech_Emergency Power System Operations via Online Feedback Optimization/figures/block_diagram_PSS.tex <==
\begin{figure}[h]
    \center
    \begin{adjustbox}{width=\columnwidth}
    \begin{tikzpicture}
        \draw[stealth-] (0,0.5) to (-.5,0.5) node[left] {$\Delta \omega$};
        \draw (0,0) rectangle +(1.5,1) node[pos=.5] {$\frac{sK_{PSS}}{1+sT}$};
        \draw[-stealth] (1.5,0.5) to (2,0.5);
        \draw (2,0) rectangle +(1.5,1) node[pos=.5] {$\frac{1+sT_1}{1+sT_3}$};
        \draw[-stealth] (3.5,0.5) to (4,0.5);
        \draw (4,0) rectangle +(1.5,1) node[pos=.5] {$\frac{1+sT_2}{1+sT_4}$};
        \draw[-stealth] (5.5,0.5) to (7.5,0.5) node[right] {$v_{pss}$};
        
        \draw (6.55,-0.2) to (6.35,-0.2) node[left, font=\footnotesize] {$-H_{lim}$};
        \draw (6.95,1.2) to (7.15,1.2) node[right, font=\footnotesize] {$H_{lim}$};
        \draw (6.55,-0.2) to (6.95,1.2);
    \end{tikzpicture}
    \end{adjustbox}
    \caption{Block diagram of the power system stabilizer.}
    \label{fig:PSS}
\end{figure}

==> 2023_PowerTech_Emergency Power System Operations via Online Feedback Optimization/figures/block_diagram_excitation.tex <==
\begin{figure}[h]
    \center
    \begin{adjustbox}{width=0.9\columnwidth}
    \begin{tikzpicture}
        \draw (-0.75,0.5) to (-1.5,0.5) node[left] {$\frac{E_{f0}}{K_{ex}}$};
        \draw[stealth-] (-1,-0.25) to (-1.5,-0.25) node[left] {$\Delta v$};
        \draw (-0.75,-1) to (-1.5,-1) node[left] {$v_{pss}$};
        
        \draw (-0.75,-0.25) circle [radius=0.25] node {$+$};
        
        \draw[-stealth] (-0.75,-1) to (-0.75,-0.5);
        \draw[-stealth] (-0.75,0.5) to (-0.75,0);
        
        \draw[-stealth] (-0.5,-0.25) to (0,-0.25);
        \draw (0,-0.75) rectangle +(1.5,1) node[pos=.5] {$\frac{1+sT_a}{1+sT_b}$};
        \draw[-stealth] (1.5,-0.25) to (2,-0.25);
        \draw (2,-0.75) rectangle +(1.5,1) node[pos=.5] {$\frac{K_{ex}}{1+sT_e}$};
        \draw (2.75,-0.75) to (2.55,-0.95) to (2.35,-0.95) node[left, font=\footnotesize] {$E_{min}$};
        \draw (2.75,0.25) to (2.95,0.45) to (3.15,0.45) node[right, font=\footnotesize] {$E_{max}$};

        \draw[-stealth] (3.5,-0.25) to (4,-00.25) node[right] {$E_f$};
    \end{tikzpicture}
    \end{adjustbox}
    \caption{Block diagram of the excitation system.}
    \label{fig:excitation}
\end{figure}


==> 2023_PowerTech_Emergency Power System Operations via Online Feedback Optimization/figures/block_diagram_governor.tex <==
\begin{figure}[h]
    \center
    \begin{adjustbox}{width=\columnwidth}
    \begin{tikzpicture}
        \draw[stealth-] (-1,0.5) to (-1.5,0.5) node[left] {$R_gp_{m0}$};
        \draw (-0.75,0.5) circle [radius=0.25] node {$+$};
        
        \draw[-stealth] (-0.75,-1) to (-0.75,0.25);
        \draw[-stealth] (-0.5,0.5) to (0,0.5);
        \draw (0,0) rectangle +(1.5,1) node[pos=.5] {$\frac{1}{R_g}$};
        \draw[-stealth] (1.5,0.5) to (2,0.5);
        \draw (2,0) rectangle +(1.5,1) node[pos=.5] {$\frac{1}{1+sT_1}$};
        
        \draw (2.75,0) to (2.55,-0.2) to (2.35,-0.2) node[left, font=\footnotesize] {$V_{min}$};
        \draw (2.75,1) to (2.95,1.2) to (3.15,1.2) node[right, font=\footnotesize] {$V_{max}$};
        
        \draw[-stealth] (3.5,0.5) to (4,0.5);
        \draw (4,0) rectangle +(1.5,1) node[pos=.5] {$\frac{1+sT_2}{1+sT_1}$};
        \draw (5.5,0.5) to (6,0.5);
        \draw[-stealth] (6,0.5) to (6,-0);
        
        \draw (-0.5,-1) to (-1.5,-1) node[left] {$\Delta \omega$};
        
        \draw[-stealth] (-0.5,-1) to (2,-1);
        \draw (2.0,-1.5) rectangle +(1.5,1) node[pos=.5] {$-D_t$};
        \draw (3.5,-1) to (6,-1);
        \draw[-stealth] (6,-1) to (6,-0.5);
        
        \draw (6,-0.25) circle [radius=0.25] node {$+$};
        \draw[-stealth] (6.25,-0.25) to (6.75,-0.25) node[right] {$p_{GOV}$};
    \end{tikzpicture}
    \end{adjustbox}
    \caption{Block diagram of the governor model.}
    \label{fig:governor}
\end{figure}

==> 2023_PowerTech_Emergency Power System Operations via Online Feedback Optimization/figures/block_diagram_simulation_model.tex <==
\begin{figure*}[]
    \centering
    \begin{tikzpicture}[scale=0.9,every node/.style={transform shape}]
        \draw[-stealth] (-1,4) to (-1,0.5) to (-0.5,0.5) node[above] {$\omega$} to (0,0.5);
        \draw (0,0) rectangle +(1.5,1) node[pos=.5] {GOV};
        \draw[-stealth] (7,3) to (7.5,3) node[above] {$\omega$} to (8,3) to (8,5) to (-1,5) to (-1,4) to (-0.5,4) node[above] {$\omega$} to (0,4);
        \draw (0,3.5) rectangle +(1.5,1) node[pos=.5] {PSS};
        \draw[-stealth] (1.5,4) to (2,4) node[above] {$v_{pss}$} to (2.5,4);
        \draw (2.5,2) rectangle +(1.5,2.5) node[pos=.5] {AVR};
        
        \draw (0.75,2.5) circle [radius=0.25] node {$+$};
        \draw[-stealth] (-1.75,1.75) to (-0.5,1.75) node[above] {$v$} to (0.75,1.75) to (0.75,2.25) node[right] {$-$};
        \draw[-stealth] (-2,3) to (-0.5,3) node[above] {$v_{OFO}$} to (0.75,3) to (0.75,2.75);
        \draw[-stealth] (1,2.5) to (2,2.5) node[above] {$\Delta v$} to (2.5,2.5);
        
        \draw (5.5,1.0) rectangle +(1.5,3) node[pos=.5] {GEN};
        \draw[-stealth] (4,3.5) to (5,3.5) node[above] {$E_f$} to (5.5,3.5);
        \draw[-stealth] (0.75,1.75) to (4.25,1.75) to (4.25,2.5) to (5,2.5) node[above] {$v$} to (5.5,2.5);
        \draw[-stealth] (4,0.5) to (4.75,0.5) to (4.75,1.5) to (5,1.5) node[above] {$p_m$} to (5.5,1.5);
        \draw[-stealth] (7,2) to (7.5,2) node[above] {$i_{inj}$} to (9.5,2) to (9.5,1.5) to (10,1.5) node[above] {$\bm i_{inj}$} to (10.5,1.5);
        
        \draw (3.75,0.5) circle [radius=0.25] node {$+$};
        \draw[-stealth] (1.5,0.5) to (2,0.5) node[above] {$p_{GOV}$} to (2.5,0.5) to (2.5,1) to (3.75,1) to (3.75,0.75);
        \draw[-stealth] (2.75,-1.5) to (2.75,0) node[left] {$p_{OFO}$} to (2.75,0.5) to (3.5,0.5);
        \draw[-stealth] (3.75,-2) to (3.75,0) node[right] {$p_{AGC}$} to (3.75,0.25);
        % Frame
        \draw[dotted] (-1.25,-0.25) to (6.75,-0.25) node[above] {\emph{Generating unit}} to (8.25,-0.25) to (8.25,5.25) to (-1.25,5.25) to (-1.25,-0.25);
        \draw[dotted] (-0.75,-0.25) to (-0.75,-0.75) to (8.75,-0.75) to (8.75,4.75) to (8.25,4.75);
        % Outputs
        \draw[dotted] (8.5,1.5) to (9.5,1.5);
        \draw[dotted] (8.5,2.5) to (9.5,2.5) to (9.5,3);
        \draw[-stealth] (8,3) to (10,3) node[above] {$\bm\omega$} to (10.5,3);
        % Inputs
        \draw[dotted] (-2,2.5) to (-1.25,2.5);
        \draw[dotted] (-1.75,1.25) to (-1.25,1.25);
        \draw[dotted] (3.25,-1.5) to (3.25,-0.5);
        \draw[dotted] (4.25,-2) to (4.25,-0.5);
        % PF, OFO
        \draw (10.5,1) rectangle +(1.5,1) node[pos=.5] {PF};
        \draw[-stealth] (12,1.5) to (12.5,1.5) node[above] {$\bm u$} to (13,1.5);
        \draw (12.5,1.5) to (12.5,-1.25) to (-1.75,-1.25) to (-1.75,1.75);
        \draw (13,0) rectangle +(1.5,2) node[pos=.5] {OFO};
        \draw (14.5,0.5) to (15,0.5) node[above] {$\bm p_{OFO}$} to (15.5,0.5) to (15.5,-1.5) to (2.75,-1.5);
        \draw (14.5,1.5) to (15,1.5) node[above] {$\bm v_{OFO}$} to (15.75,1.5) to (15.75,-1.75) to (-2,-1.75)  to (-2,3);
        % AGC
        \draw (10.5,2.5) rectangle +(1.5,1) node[pos=.5] {AGC};
        \draw (12,3) to (12.5,3) node[above] {$\bm p_{AGC}$} to (16,3) to (16,-2) to (3.75,-2);
        % Dots
        \filldraw[black] (0.75,1.75) circle (1pt);
        \filldraw[black] (-2,2.5) circle (1pt);
        \filldraw[black] (-1.75,1.25) circle (1pt);
        \filldraw[black] (-1,4) circle (1pt);
        \filldraw[black] (8,3) circle (1pt);
        \filldraw[black] (9.5,1.5) circle (1pt);
        \filldraw[black] (9.5,3) circle (1pt);
        \filldraw[black] (12.5,1.5) circle (1pt);
        \filldraw[black] (3.25,-1.5) circle (1pt);
        \filldraw[black] (4.25,-2) circle (1pt);
        
    \end{tikzpicture}
    %\end{adjustbox}
    \caption{Block diagram of the dynamic power system simulator \emph{DynPSSimPy} including the OFO controller. The blocks PSS, AVR, GOV, GEN, AGC, PF and OFO correspond to the power system stabilizer, the automated voltage regulator, the governor, the synchronous machine, the excitation system, the power flow equations and the OFO controller, respectively. The blocks corresponding to one generating unit are grouped by the dotted frame, and possible additional generation units are indicated by the second dotted frame.}
\label{fig:simulation_model}
\end{figure*}
